ChatBI: Towards Natural Language to Complex Business Intelligence SQL

The Natural Language to SQL (NL2SQL) technology provides non-expert users who are unfamiliar with databases the opportunity to use SQL for data analysis.Converting Natural Language to Business Intelligence (NL2BI) is a popular practical scenario for NL2SQL in actual production systems. Compared to NL2SQL, NL2BI introduces more challenges. In this paper, we propose ChatBI, a comprehensive and efficient technology for solving the NL2BI task. First, we analyze the interaction mode, an important module where NL2SQL and NL2BI differ in use, and design a smaller and cheaper model to match this interaction mode. In BI scenarios, tables contain a huge number of columns, making it impossible for existing NL2SQL methods that rely on Large Language Models (LLMs) for schema linking to proceed due to token limitations. The higher proportion of ambiguous columns in BI scenarios also makes schema linking difficult. ChatBI combines existing view technology in the database community to first decompose the schema linking problem into a Single View Selection problem and then uses a smaller and cheaper machine learning model to select the single view with a significantly reduced number of columns. The columns of this single view are then passed as the required columns for schema linking into the LLM. Finally, ChatBI proposes a phased process flow different from existing process flows, which allows ChatBI to generate SQL containing complex semantics and comparison relations more accurately. We have deployed ChatBI on Baidu's data platform and integrated it into multiple product lines for large-scale production task evaluation. The obtained results highlight its superiority in practicality, versatility, and efficiency. At the same time, compared with the current mainstream NL2SQL technology under our real BI scenario data tables and queries, it also achieved the best results.

==> 4.impl.tex <==
\section{Implementation}\label{sec:impl}

==> bo.tex <==
The Bayesian Optimization method introduces exploration, and the parallelism of the acquisition function selection is usually larger in confidence if it is far from the nearest sample point and is considered an aggressive exploration. 
The online tuning scenario wants to avoid aggressive exploration, and ContTune introduces the general methods that are efficient for one-shot tuning as conservative exploration. 
ContTune designs a new acquisition function to determine whether to use the parallelism chosen by the Bayesian Optimization method or general methods based on the distance of the parallelism chosen by the Bayesian Optimization method to the nearest sample point and the distance to the nearest sample point is closely related to the confidence level, which compensates the limitation of using only the mean value in the Bayesian Optimization method (Section 6.1). 
The \textit{Bayesian Optimization method}, \textit{general methods}, and the \textit{acquisition function} make up conservative Bayesian Optimization.



These works ~\cite{gulisano2012streamcloud,lohrmann2015elastic,fu2017drs,zaharia2013discretized,fischer2015machines,googleCloudDataflow2016,kalavri2018three,mei2020turbine,liu2022dragster} can be regarded as a tune using  \textit{multi-operator} pattern, and \textit{single-operator} pattern works ~\cite{castro2013integrating,heinze2014latency,xu2016stela,floratou2017dhalion,pravega2017,gedik2013elastic}. 
By the way, ContTune can use the $St_{samples}$ of other unchanged operators after some operators are changed because the tune using \textit{multi-operator} pattern is only related to tuned operator itself. 
As shown in Figure ~\ref{f1}, ContTune concurrently tunes all operators at one tuning. 

\iffalse
Inspired by the fact that the one-dimensional Subspaces Bayesian Optimization method will have better optimization results ~\cite{kirschner2019adaptive} and that horizontal tuning (tuning the parallelism of operator) has a greater improvement on the processing ability of the operator than vertical tuning (not tuning parallelism, tuning other parameters) ~\cite{roger2019comprehensive,cardellini2022runtime}, ContTune uses only parallelism as the One-Dimensional Subspaces for the Bayesian Optimization.
\fi

ContTune uses the performance model generated by GP and $St_{samples}$ that better solves the nonlinearity problem ~\cite{kalavri2018three,mei2020turbine,liu2022dragster} encountered in the current state-of-the-art methods ~\cite{kalavri2018three,mei2020turbine} of one-shot tuning.


\begin{equation}
\label{UCB}
x_t=arg\max _{x\in D}\left( \mu _{t-1}\left( x \right) +\beta ^{1/2}\sigma _{t-1}\left( x \right) \right) 
\end{equation}
LCB ~\cite{liu2014gaspad}, 
\begin{equation}
\label{LCB}
x_t=arg\max _{x\in D}\left( \mu _{t-1}\left( x \right) -\beta ^{1/2}\sigma _{t-1}\left( x \right) \right) 
\end{equation}
and EIC ~\cite{gelbart2014bayesian}, 
\begin{equation}
\begin{gathered}
\label{EIC}
y\left( x \right) \sim GP\left( \mu \left( x \right) ,k\left( x,x \right) \right) \\
PR\left( x,W \right) =P\left( y\left( x \right) \ge W \right) \\
x_t=arg\max _{x\in D}\left( \left( x^*-x \right) \times PR\left( x,W \right) \right) 
\end{gathered}
\end{equation}
and $x^*$ means the minimum parallelism that its corresponding processing ability is lager than current workload $W$ in $St_{samples}$. 
for the selection of the acquisition function in Bayesian Optimization. They all have certain problems.
For UCB, the processing ability of the operator is represented by the mean value plus the confidence level, which encourages the use of parallelism smaller than the target parallelism and tends to make job backpressure. 
For LCB, the processing ability of the operator is represented by the mean value minus the confidence level, which encourages the use of parallelism larger than the target parallelism and can result in a waste of CPU resources. 
EIC shows a certain chance of encouraging the exploration of parallelism less than the target parallelism, and once these parallelisms are attempted, additional reconfigurations are required to keep the job from backpressure. 

Formally, our acquistion function is:
\begin{equation}
\begin{gathered}
\label{OUR}
I\left( x \right) =\begin{cases}
	1&		if\ x\ge 0\\
	0&		if\ x<0\\
\end{cases} \\
x_t=arg\max _{x\in D}\left( x^*-x \right) I\left( \mu \left( x \right) -W \right) 
\end{gathered}
\end{equation}
and $x^*$ means the minimum parallelism that its corresponding processing ability is larger than current workload $W$ in $St_{samples}$. 
ContTune uses Bayesian Optimization as exploitation. 
